SEA: Graph Shell Attention in Graph Neural Networks

A common issue in Graph Neural Networks (GNNs) is known as over-smoothing. By increasing the number of iterations within the message-passing of GNNs, the nodes' representations of the input graph align with each other and become indiscernible. Recently, it has been shown that increasing a model's complexity by integrating an attention mechanism yields more expressive architectures. This is majorly contributed to steering the nodes' representations only towards nodes that are more informative than others. Transformer models in combination with GNNs result in architectures including Graph Transformer Layers (GTL), where layers are entirely based on the attention operation. However, the calculation of a node's representation is still restricted to the computational working flow of a GNN. In our work, we relax the GNN architecture by means of implementing a routing heuristic. Specifically, the nodes' representations are routed to dedicated experts. Each expert calculates the representations according to their respective GNN workflow. The definitions of distinguishable GNNs result from k-localized views starting from the central node. We call this procedure Graph Shell Attention (SEA), where experts process different subgraphs in a transformer-motivated fashion. Intuitively, by increasing the number of experts, the models gain in expressiveness such that a node's representation is solely based on nodes that are located within the receptive field of an expert. We evaluate our architecture on various benchmark datasets showing competitive results compared to state-of-the-art models.

==> _appx.tex <==
\section{Results - switch layer on different positions}

\begin{table}[!h]
    \centering
    \begin{tabular}{c|c|c|c}
        Method & AUC(\%) & \# parameters & \#experts \\
        \toprule
        % Test ROC:  {'rocauc': 0.8031711697792541}  
        Vanilla & 80.31 & 384 701 & 10\\
        %
        %{'rocauc': 0.7895614052028815}
        Switch Layer Post-Head &  78.95 & 996 761 & 10 \\
        %
        %{'rocauc': 0.7740879507136098}
        Switch Layer Pre-Head & 77.40 & 2 881 421 & 10\\
        %
        % {'rocauc': 0.7320033218100003} 
        Switch Layer Post-Attention & 73.20 & 1 608 821 & 10\\
        %
        % {'rocauc': 0.7102879545761794}
        % but extreme high variance 
        Switch Layer Pre-Attention  & 71.02 & 1 608 821 & 10\\
        %
        % Test ROC:  {'rocauc': 0.748101546959192} 
        Shell Model (separated) - MHA & 74.81 & 750 119 & 3 \\
        % Test ROC:  {'rocauc': 0.7514436354506655}
        Shell Model (separated) - MHA-Switch & 75.14 & & 3\\
        %
        %Test ROC:  {'rocauc': 0.760595028872709}
        Shell Model (overlap) - Switch & 76.05 & & 3\\
    \end{tabular}
    \caption{Results on MolHIV}
    \label{tab:my_label}
\end{table}




\begin{table*}
%    \centering
\begin{minipage}[t]{0.49\textwidth}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c|c|c}
        Method & AUC(\%) & \# parameters & \#experts \\
        \toprule
        \midrule
        GCN+{\small \textsc{GraphNorm}}[$\dagger$] & 78.83 & 526K & -\\
        GIN & & & -\\
        Graphormer-{\small \textsc{Flag}}[$\dagger$] & 80.51 & 47.0M & -\\
        DGN[$\diamond$] & 79.05 & & -\\
        SAN[$\diamond$] & 77.85 & &- \\
        \midrule
        % Test ROC:  {'rocauc': 0.7806717008825973} 
        Vanilla GTL & 78.06 & 428 551 & 4\\
        % Test ROC:  {'rocauc': 0.7892350180575136} 
        Graph Shell Attention (\#1) & 78.92 & 591 767 & 4\\
        % Test ROC:  {'rocauc': 0.8007029876977153}
        Graph Shell Attention (\#2) & 80.07 & 836 591 & 4\\
        % Test ROC:  {'rocauc': 0.786913613627146}
        Graph Shell Attention (\#3) & 78.69 & 836 591 & 4
    \end{tabular}
}
    \caption{Results on MolHIV; [$\dagger$]: \cite{ying2021_graphormer}; [$\diamond$]:\cite{kreuzer_2021_rethinking}}
    \label{tab:molhiv}
    \end{minipage}
    \begin{minipage}[t]{0.49\textwidth}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{c|c|c|c}
        Method & AUC(\%) & \# parameters & \#experts \\
        \toprule
        \midrule
        %GCN+{\small \textsc{GraphNorm}}[$\dagger$] & & - & -\\
        %GIN & & & -\\
        Graphormer-{\small \textsc{Flag}}[$\dagger$] & 31.39 & 119.5M & -\\
        DGN[$\diamond$] & 28.85 & 6.7M & -\\
        \midrule
        %SAN[$\diamond$] & & &- \\
        %Test:  {'ap': 0.24414809837226212}
        Vanilla GTL & 24.41 & & \\
        Graph Shell Attention (\#1) & 14.11 & & \\
        Graph Shell Attention (\#2) & 24.48 & & \\
        Graph Shell Attention (\#3) & 24.27 & &
    \end{tabular}
}
    \caption{Results on MolPCBA; [$\dagger$]: \cite{ying2021_graphormer}; [$\diamond$]:\cite{kreuzer_2021_rethinking}}
    \label{tab:molpcba}
\end{minipage}
\end{table*}


\begin{table*}
%\centering
\begin{tabular}{c|c|c|c}
        Method & MAE & \# parameters & \#experts \\
        \toprule
        \midrule
        GCN[$\diamond$] & 0.367 & -\\
        GIN[$\diamond$] & 0.526 & & -\\
        GAT[$\diamond$] & 0.384 & & \\
        %
        SAN[$\diamond$] & 0.139 & &- \\
        \midrule
        Vanilla GTL & 0.182 & & \\
        Graph Shell Attention (\#1) & &  & \\
        Graph Shell Attention (\#2) & & & \\
        Graph Shell Attention (\#3) & 0.181 & & 
    \end{tabular}
    \caption{Results on ZINC; [$\diamond$]:\cite{kreuzer_2021_rethinking}}
    \label{tab:molpcba}
\end{table*}


==> _notes.tex <==
\begin{definition}[Local-instance Structure]
The local-instance structure refers to the local pairwise similarity between different instances. To preserve the local-instance structure of graph-structured data, a pair of similar graphs/subgraphs, $\mathcal{G}$ and $\mathcal{G}'$, are expected to be mapped to the nearby positions of embedding space, while the dissimilar pairs should be mapped to far apart.
\end{definition}

\begin{definition}[Global-semantic Structure]
A real-world dataset is usually distributed as different semantic clusters. Therefore, we define the global-semantic structure of a dataset as the distribution of its semantic clusters, and each cluster is represented by a prototype (i.e., a representative cluster embedding). Since the semantics of a set of graphs can be structure in a hierarchical way, we represent the whole dataset with hierarchical prototypes. 
\end{definition}

==> _tab_dataset_metrics.tex <==
\definecolor{gold}{RGB}{212, 175, 55}
\definecolor{silver}{RGB}{170, 169, 173} 
\definecolor{bronze}{RGB}{176, 141, 87} 
\newcolumntype{Y}{>{\centering\arraybackslash}p{2.5cm}}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}

\newcommand{\gold}[1]{\cellcolor{gold}{\bfseries #1}}
\newcommand{\silver}[1]{\cellcolor{silver}{\bfseries #1}}
\newcommand{\bronze}[1]{\cellcolor{bronze}{\bfseries #1}}

\begin{table*}
\centering
%\begin{minipage}[t]{0.75\textwidth}
%\resizebox{1\linewidth}{!}{
\begin{tabular}{|c| YY|HYY|YY|}
        \toprule
        & \multicolumn{2}{c}{\bfseries ZINC} & {\bfseries MOLPCBA} & \multicolumn{2}{c}{\bfseries OGBG-MOLHIV} & \multicolumn{2}{c}{\bfseries PATTERN}\\
        \bottomrule
        \blackcell{Model} & \blackcell{\#params.} & \blackcell{MAE} & \blackcell{\% ACC} & \blackcell{\#params.} & \blackcell{\%ROC-AUC} & \blackcell{\#params.} & \blackcell{\% ACC}  \\
        \toprule
        GCN~\cite{Kipf_gcn_2017} & 505K & 0.367 & & & 76.06 & & 71.892\\
        GIN~\cite{Xu_gin_2018} & & 0.526 & & & - & & \silver{85.590}\\
        GAT~\cite{velickovic_gat_2017} & & 0.384 & & - & - & - & 78.271\\
        SAN~\cite{kreuzer_2021_rethinking}& - & \silver{0.139} & - & - & 77.85 & - & \gold{86.581}\\
        DGN~\cite{Beaini_dgn_2020} & - & - & 28.85 & - & \bronze{79.05} & - & -\\
        Graphormer-{\small \textsc{Flag}}/-{\small \textsc{Slim}}~\cite{ying2021_graphormer} & - & \gold{0.122} & 31.39 & - & \gold{80.51} & - & -\\
\midrule
        % 
        %% REFERS TO ZINC FULL dataset
        %
        % Vanilla GTL & 0.143 & 24.41 & 78.06 &\\
        % Graph Shell Attention (\#1) & \gold{0.115} & 14.11 & 78.92 &\\
        % Graph Shell Attention (\#2) & 0.212 & 24.48 & \silver{80.07} &\\
        % Graph Shell Attention (\#3) & 0.159 & 24.27 & 78.69 &\\
        % \bottomrule
        Vanilla GTL & - & 0.200 & 24.41 & - & 78.06 & - & 81.350\\
        GTL-\textsc{$2$-hop} & - & 0.195 & - & - & - & - & -\\
        %Graph Shell Attention (\#1) & (0.449/0.483) & 14.11 & 78.92 & 54.834\\
        SEA-GNN & - & \bronze{0.185} & 24.48 & - & \silver{80.07} & - & 78.601\\
        SEA-GNN-\textsc{aggregated} & - & 0.246 & 24.27 & - & 78.69 & - & \bronze{82.065}\\
        SEA-GNN-\textsc{$2$-hops} & - & (-/-) & - & - & - & - & -\\        \bottomrule
    \end{tabular}
%}
    \caption{Comparison to state-of-the art on benchmark datasets from \cite{hu_2020_ogb} (ogbg-molhiv), ZINC \cite{irwin_zinc_2012}, and PATTERN; results are partially taken from \cite{kreuzer_2021_rethinking, dwivedi_2020_benchmarking}; color coding (gold/silver/bronze)};
    \label{tab:sea_comparison}
%\end{minipage}
\end{table*}


==> _tikz_GraphTransformerLayer.tex <==
\tikzset{%
  outerblock/.style    = {draw, dotted, thick, rectangle, minimum height = 5cm,
    minimum width = 9cm},
  innerblock/.style    = {draw, thick, rectangle, minimum height = 3em,
    minimum width = 3em},
  sum/.style      = {draw, circle, node distance = 2cm}, % Adder
  input/.style    = {coordinate}, % Input
  output/.style   = {coordinate}, % Output
  textblock/.style={rectangle,draw, fill=gray!10, minimum width=3cm, minimum height=0.5cm, rounded corners=0.8ex, anchor=center, inner sep=0},
  textblock_red/.style={rectangle,draw,fill=red!20,rounded corners=.8ex},
}

\definecolor{lavander}{cmyk}{0,0.48,0,0}
\definecolor{violet}{cmyk}{0.79,0.88,0,0}
\definecolor{burntorange}{cmyk}{0,0.52,1,0}
\definecolor{blue}{cmyk}{0.8,0.4,0.4,0}
\definecolor{green}{cmyk}{0.8, 0.0, 0.6, 0}

\def\lav{lavander!90}
\def\oran{orange!30}
\def\blue{blue!30}
\def\green{green!30}

\tikzstyle{one_hop}=[draw, circle, 
violet, 
bottom color=\lav, 
top color= white, 
text=violet, minimum width=10pt]
\tikzstyle{superpeers}=[draw, circle, burntorange, left color=\oran, text=violet, minimum width=10pt]
\tikzstyle{two_hop}=[draw, circle, blue, bottom color=\blue, top color= white, text=violet, minimum width=10pt]

\tikzstyle{legend_general}=[rectangle, rounded corners, thin, burntorange, fill= white, draw, text=violet, minimum width=2.5cm, minimum height=0.8cm]
\tikzstyle{legend_general_pos}=[rectangle, rounded corners, thin, green, fill= white, draw, text=violet, minimum width=2.5cm, minimum height=0.8cm]
\tikzstyle{legend_general_neg}=[rectangle, rounded corners, thin, red, fill= white, draw, text=violet, minimum width=2.5cm, minimum height=0.8cm]
\tikzstyle{module}=[rectangle, rounded corners, thin, blue, fill= white, draw, text=blue, minimum width=2.0cm, minimum height=0.8cm]
\tikzstyle{module_neg}=[rectangle, rounded corners, thin, red, fill= white, draw, text=blue, minimum width=2.0cm, minimum height=0.8cm]
                           
\begin{tikzpicture}[auto, thick, node distance=0.75cm]

\begin{scope}
\node[draw, fill=blue!10, dotted, rectangle, minimum width=9cm, minimum height=6cm, rounded corners=1ex] at (3.5,2.5) {};

\node[textblock, minimum width=1cm, fill=gray!20] (hi) at (0,-1.5) {$h_i$};
\node[textblock, minimum width=1cm, fill=gray!20] (hj) at (4.5,-1.5) {$h_j$};


\node[textblock, minimum width=1cm, fill=cyan!20] (Q) at (0,0) {$Q$};
\node[textblock, minimum width=1cm, fill=cyan!20] (K) at (3,0) {$K$};
\node[textblock, minimum width=1cm, fill=cyan!20] (V) at (6,0) {$V$};
\node[textblock] (product) at (1.5,1.5) {Product};
\node[textblock] (scaling) at (1.5,2.5) {Scaling};
\node[textblock, fill=green!20] (softmax) at (1.5,3.5) {softmax};
\node[circle, draw] (dot) at (6, 3.5) {};
\node[textblock] (sum) at (6,4.5) {sum};
\node[textblock] (concat) at (3,6) {Concat};
\node[textblock, fill=cyan!20] (linear1) at (3,7) {Linear};
\node[textblock, fill=red!20] (addnorm1) at (3,8) {Add \& Normalization};
\node[textblock, fill=cyan!20] (linear2) at (3,9) {Linear};
\node[textblock, fill=red!20] (addnorm2) at (3,10) {Add \& Normalization};

\draw[->] (Q) -- (0, 0.75) -- (1, 0.75) -- (product);
\draw[->] (K) -- (3, 0.75) -- (2, 0.75) -- (product);
\draw[->] (product) -- (scaling);
\draw[->] (scaling) -- (softmax);
\draw[->] (softmax) -- (dot);
\draw[->] (dot) -- (sum);
\draw[->] (sum) -- (6,5) -- (4,5) -- (concat);
\draw[->] (concat) -- (linear1);
\draw[->] (linear1) -- (addnorm1);
\draw[->] (addnorm1) -- (linear2);
\draw[->] (linear2) -- (addnorm2);

\draw[->] (V) -- (dot);


\draw[->] (hi) -- (Q);
\draw[->] (hj) -- (4.5, -0.75) -- (3, -0.75) -- (K);
\draw[->] (hj) -- (4.5, -0.75) -- (6, -0.75) -- (V);

\draw[->] (0, -0.75) -- (-1.5, -0.75) -- (-1.5, 8) -- (addnorm1);
\draw[->] (3, 8.5) -- (-1.5, 8.5) -- (-1.5, 10) -- (addnorm2);

\end{scope}


\end{tikzpicture}
